The Missing Piece in Complex Analytics: Low Latency, Scalable Model Management and Serving with Velox

To support complex data-intensive applications such as personalized recommendations, targeted advertising, and intelligent services, the data management community has focused heavily on the design of systems to support training complex models on large datasets. Unfortunately, the design of these systems largely ignores a critical component of the overall analytics process: the deployment and serving of models at scale. In this work, we present Velox, a new component of the Berkeley Data Analytics Stack. Velox is a data management system for facilitating the next steps in real-world, large-scale analytics pipelines: online model management, maintenance, and serving. Velox provides end-user applications and services with a low-latency, intuitive interface to models, transforming the raw statistical models currently trained using existing offline large-scale compute frameworks into full-blown, end-to-end data products capable of recommending products, targeting advertisements, and personalizing web content. To provide up-to-date results for these complex models, Velox also facilitates lightweight online model maintenance and selection (i.e., dynamic weighting). In this paper, we describe the challenges and architectural considerations required to achieve this functionality, including the abilities to span online and offline systems, to adaptively adjust model materialization strategies, and to exploit inherent statistical properties such as model error tolerance, all while operating at "Big Data" scale.

==> results.tex <==
%!TEX root = veloxms.tex


\section{The Velox Prototype}

% We have implemented a prototype of \system to serve and update recommendendations
% using collaborative filtering.
Although \system is in the early stages of development,
we have a fully functioning prototype of a collaborative filtering based recommender
system. \system reads models from Tachyon and serves point predictions, top-k, and the
best item from a user-provided base set. \system can also update user models as described,
implementing a closed form solution for incremental updates to a regression model \dan{I have no idea if this is correct. But we should say something about the updates algorithm}.
In the current implementation, all \vsets are explicit, although this is simply an
artifact of implementing a recommendation system, and not indicative of the difficulty
of implementing implicit \vsets. Right now, \system implements a shared nothing architecture.
This means that although it is distributed, we have not implemented any of the shared
strategies as described above.

Users can interact with the \system prototype via HTTP using a RESTful interface and JSON.
Using our prototype, we have run a few experiments to validate our initial design decisions
and understand the baseline performance characteristics.

The first experiment looked at the effect of model complexity on prediction latency. In
this experiment, \system was running on a single node co-located with all \vsets to isolate
the effect of model complexity on prediction latency. We varied the complexity
of the model by changing the number of factors in the models (\ie the length of the feature
vectors). We expect model size to have a linear relationship to prediction latency,
as the dominant cost in this experiment is computing the inner-product of the user and item
models, which is $\BigO{\# \text{factors}}$. To further tease apart the effects of
model size, we varied the number of predictions by requesting the
top-ranked item from a user-provided subset of the items, varying the
size of the base item subset. The results of this experiment can be seen
in \figref{fig:predict-latency}. Also included in these results are the
effect of caching predictions (in-memory in Tachyon -- the underlying
storage layer -- not in the \system heap). Predictions are constant size
regardless of the size of the model used to generate them. As expected,
latency increases linearly as both the number of predictions increases
and as the size of the model increases. These results clearly demonstrate
the performance benefits that caching can provide, particularly when models
get large.
\dan{probably want to split these results into a couple graphs, one that compares
  prediction performance as base itemset gets bigger across a couple model sizes,
  and one that compares prediction latency as a function of model size for a couple
itemset sizes. Important to demonstrate both linear relationships}

Our second experiment investigated the effect of model size on
the cost (latency) of online model updates. The algorithm for online updates is cubic
in the size of the model, so we expect to see the models get significantly more
expensive to update as the number of factors increases. The results for this experiment
can be seen in \figref{fig:update-latency}.




\begin{figure}[t]
\includegraphics[width=\linewidth]{data/online_update_latency_results}
\vspace{0pt} % yes, this has an effect
\caption{\textbf{Update latency vs model complexity}
\vspace{-1em}
}
\label{fig:update-latency}
\end{figure}


==> scratch.tex <==
% By combining vast amounts of data with recent developments in sophisticated statistical modeling techniques we have created the opportunity to build systems which can learn from data to automatically improve user experience respond to changes in


% For matrix factorization methods, a common class of modeling techniques founds within recommender systems, we explore a hybrid approach to offline and online learning.
% We enable the


% For a common class of modeling tasks found within recommender systems, we explore support for a range of new models which can be divided into offline and online learning phases.
% In particular we focus here on matrix factorization models used in the context of collaborative filtering.
% We introduce support for incremental updates to these models by recomputing user features based on new signal.


% Paragraph 1: Machine learning is widely used. From generating playlists for Internet Radio to automatically detecting supernovae in astronomic surveys, machine learning provides a way
% for us to automatically model processes in our world in a principled way.
%
% Paragraph two: Historically, the focus has been on training models, and what happens to models after they have been trained has been neglected.
%
% Paragraph three: Increasing use of class of models that necessitate both offline (high latency acceptable) learning and online learning (must adapt to changing user behavior in real-time or in seconds, thus no time to retrain general model to reflect new user behavior), and that require low-latency high-throughput predictions on model requires a principled approach to model-serving.
%
% Paragraph four?: Example use case for model-serving (Pandora). General model of user behavior. Several learned models representing different \eg "moods", must quickly decide what model best represents user's current state to play them correct music. User "likes", "dislikes" a song, must update user's model with this additional rating. User wants to feel like radio has immediately responded to this additional info.
%
%
% Paragraph five: Requirements for model serving (sort of defining the scope of the problem). Ability to integrate with an offline training system. Serve low-latency predictions - both point predictions and top-k. Online updates to models. Manage model over lifetime (from training to online updates to detection of staleness to triggering retraining, etc). Interface? These requirements present both new challenges and opportunies for building serving systems. In the rest of this paper, we outline the design space for building model-management systems and some of the challenges involved. We then present preliminary work on a system we are developing in this space, and discuss the system design decisions we have made.




\section{Learning vs Prediction}

Summary of the differences between offline training of a model and making predictions using that model.

\subsection{What is a model and where does it come from?}

\dan{Leave section for Joey}


\section{Learning vs Prediction}



Machine learning ubiquitous today (lots of examples). Systems for machine learning are now commonplace in systems conferences.
Historically, the hard problem in machine learning has been considered to be training models. Often requires several passes over a large dataset, IO intensive, hyper-parameter tuning, cross-validation, etc. We have seen a lot of successes in this area (e.g. Spark, GraphLab, HogWild, Mahout...).

However, this focus on training is only half the story to building systems for practical/applied machine learning. There are several classes of models/applications that require low-latency predictions (\eg for choosing content when serving webpages) and that must react in real-time to the actions of a user (online learning).

Example one:
personalized content on the web (Pandora, Netflix, Amazon)

Example two: real-time directions with traffic/road condition awareness



Applied machine learning - using statistical models to make practical predictions about the world - has become ubiquitous over the last few years.
From use cases as diverse as generating playlists for personalized internet radio to automatically detecting supernovae in astronomy surveys to providing real-time automated language translation, machine learning is being used to automate and improve the efficiency of processes in many different domains.
Developing a machine learning application has three stages.
The first stage is selecting an appropriate model for the domain and determining the best set of features to represent data points in your domain (the development stage).
Typically, an expert (\eg data scientist) experiments with many models and features, testing each one on some representative sample of the data (often with a known right answer) until she makes a decision on which model and set of features to use.
The second stage is to learn the best parameters of this model on the actual data set in use, often by finding the minimum of some cost function using an optimization algorithm (the training stage).
This stage tends to be very resource intensive and can take a long time, especially if the dataset is large and the optimization algorithm needs to make many passes over the dataset.
The final stage is using the model to make predictions on new data (the prediction stage).
Compared to the cost of training a model, making a single prediction tends to be very cheap.
Indeed, much of the practical power of machine learning stems from being able to invest significant computational resources up front during training to get a cheap way to make accurate predictions later (\eg as part of a user-facing application that must respond in real-time).
These predictions generally take one of two forms.
It can be a point prediction, where given a piece of data the model predicts a category (classification) or score (regression) for that piece of data --- for example, given a movie, a model of a user may predict the score the rating the user will give that movie.
Or it can be a top-$k$ prediction, where the model attempts to predict the top-$k$ data items for a model --- continuing with the movie example, a user-model may be asked to predict the 10 movies that a user is most likely to enjoy.

% TODO could put a diagram in here showing the closed loop relationship between training and predictions to better illustrate the end to end pipeline

Historically, the focus of both the machine learning community and the systems community has been on developing more efficient ways to train models.
\dan{Sentence here about the focus of the ML community, highlight some of the significant successes}.
And the systems community has been drawn to training as the most resource intensive part of a machine learning application, developing a variety of approaches for speeding up machine learning through parallelization, distributing the learning over a cluster, and exploiting new hardware trends (\eg GPUs, RDMA, etc), with considerable success (cite Mahout, GraphLab, Spark, Stratosphere, etc.).

Much less attention has been paid to the prediction stage, and more broadly to developing systems to manage a model (or \emph{data product}) after it has initially been trained.
Two complementary trends suggest that it's time to investigate the right way to build model-management systems.
The first is the increasing use of machine learning on the fast path for serving user-facing queries.
Many companies have bet their business models on personalization, being able to tailor each individual's user-experience on their website using machine learning techniques like collaborative filtering to provide personalized recommendations.
This means that predictions need to be made for every web-page served (often tens or hundreds of predictions per page).
The second trend is the increasing desire to make online updates to personalized models at a much lower latency than is possible when retraining the models on the full dataset.
Instead, these use cases would like to take users most recent actions (those after the model has been trained) into account when making predictions, as it is these most recent actions that can carry the most predictive power when making accurate predictions.

For example, \dan{Walk through an example use case/motivating story here}

In this paper, we examine the system requirements needed to build a machine-learning model-management system.
We then discuss the technical challenges involved in building such a system --- particularly in the context of the database data-serving literature --- and explore some opportunities that building this new type of system affords us.
Finally, we present the preliminary work on \system, a model serving system we are building, and some of the early lessons learned.






% \textbf{Latent Factor Models}



% \textbf{Recommender Systems}  A popular class of data-products are recommender systems which target content to individuals by combining behavioral data (\eg ratings and clicks) with data describing users (\eg demographics), the items being considered (\eg content descriptions) and the context (\eg search queries).
% Although there are many variations on the underlying model structure the majority of the recent developments have adopted a form of matrix factorization.

% Matrix factorization models express the affinity of user for a particular item as a real valued score (\ie rating).
% These models associate a latent factor $w_u \in \reals^d$ with each user $u$ and $x_i \in \reals^d$ with each item $i$.
% The affinity of user $u$ has for item $i$ is then modeled as:
% \[
%   \text{affinity}(u,i) = w_u^T x_i +  \epsilon_{u,i}
% \]
% for some noise term $\epsilon_{u,i} \sim N(0,\sigma^2)$.
% While additional features may be used to capture knowledge about the user (\eg age) and the item (\eg genre) we restrict our attention to this simple model since it captures all the systems ideas in the later sections.

% Given observations about user affinities for a particular set of items we can infer the factors by solving the following optimization problem:
% \[
%   (w,x) = \arg \min_{w,x} \sum_{(u,i) \in \text{Obs}}
%   \left( r_{ui} - w_u^T x_i  \right)^2 + \lambda \left(||w||_2^2 + ||x||_2^2 \right)
% \]
% This is typically accomplished offline by applying iterative algorithms such as Alternating Least Squares or stochastic gradient descent.
% Once the latent factors have been compute, the user rating for a particular time can be predicted by evaluating the inner product $w_u^T x_i$ for a user $u$ and item $i$.


% \subsection{Personalized Prediction Service}

% Personalized predictions services (\eg spam classification or personalized search) attempt to learn specialized models for individuals or tasks.
% For example in spam classification each user might have different interpretation of what represents spam.
% Alternatively, in personalized search the relevance of content may differ across individuals.



% While recommender systems could be viewed as a form of personalized prediction services, they are often treated separately due to the introduction of co

% These services broadly employ range of multitask learning techniques which allows the system to generalize knowledge across users.
% For example, individual


% In contrast these models

% In many ways personalized prediction services share many common properties with recommender systems.






% Associated with each user $u$ and item $i$ are latent factors $w_u \in \mathbb{R}^d$ and $x_i \in \mathbb{R}^d$.
% The affinity of user $u$ has for item $i$ is then modeled as:
% \[
%   \text{affinity}(u,i) = w_u^T x_i  + \epsilon_{u,i}
% \]
% for $\epsilon_{u,i} \sim N(0,\sigma^2)$.

% Both the user factor $w_u$ and item factors $x_i$ are learned from data a




% While additional features may be used to capture knowledge about the user (\eg age) and the item (\eg genre) we restrict our attention to this simple model since it captures all the systems ideas in the later sections.



% If feature information is available



% \subsection{The Learning Model Abstraction}

% While there are a wide range of models in the machine learning literature, for the initial design of Velox we restrict our attention to the simple yet expressive family of generalized linear models (GLM) with feature transformations.
% A model in Velox is a function from some input features $x \in \mathcal{X}$ (\eg the information describing a song or credit card transaction) to a prediction $y \in \mathbb{R}$ (\eg a users rating for the song or the probability that the transaction is fraudulent) with the following form:
% \begin{equation}
% g(w^T f(x, \theta) ) \rightarrow y \label{eqn:glm}
% \end{equation}
% Each model is parameterized by a $d$-dimensional weight vector $w \in \mathbb{R}^d$.
% The feature transformation function $f: \mathcal{X} \rightarrow \mathbb{R}^d$
% maps $x \in \mathcal{X}$ (\eg a movie id, text, or an image) into a $d$-dimensional vector space and is parameterized by a potentially large number of parameters $\theta$ which we will discuss shortly.
% The linear nature of the GLM derives from the linear combination of the transformed feature space.
% Finally the function $g: \mathbb{R} \rightarrow \mathbb{R}$ permits scaling and non-linear transformations of the prediction output and is used in classification tasks.



% This simple yet powerful abstraction is sufficient to express a wide range of models and yet also isolates the key elements that are relevant to the design of the Velox system.
% The GLM abstraction embodies the predictive structure of a range of commonly used models including support vector machines, linear regression, and logistic regression.
% In following we present two common modeling applications and review their embedding in the GLM abstraction and how this effects the design of the Velox system.



% \subsection{Recommender Systems}

% A popular class of data-products are recommender systems which target content to individuals by combining behavioral data (\eg ratings and clicks) with data describing users (\eg demographics), the items being considered (\eg content descriptions) and the context (\eg search queries).
% While there are many variations on the underlying model the majority of the recent developments have adopted a form of matrix factorization.


% Expressed in the context of the GLM framework
% Expressed in the context of the GLM framework, a separate weight (model) $w_u \in \mathbb{R}^d$ is learned for each users $u$.


% Meanwhile the feature transformation $f(\cdot, \theta)$ and parameters $\theta$ characterizing


% The features $x \in \mathcal{X}$ describing each item $i$ (\eg color, price, etc...) in conjunction with ratings data are used to construct a latent feature representation $f(x_i) = \theta_i \in \mathbb{R}^d$ for each item.
% The affinity of user $u$ has for item $i$ is then modeled as:
% \[
%   \text{affinity}(u,i) = w_u^T \theta_i
% \]
% Given observations about user affinities (\eg ratings $r_{ui}$) for a particular set of items we can jointly infer the models for each user $w_u$ and the latent feature representation $\theta_i$ for each item by solving the following optimization problem:
% \[
%   (w,\theta) = \arg \min_{w,\theta} \lambda \left(||w||_2^2 + ||\theta||_2^2 \right) + \sum_{(u,i) \in \text{Obs}}
%   \left( r_{ui} - w_u^T \theta_i  \right)^2
% \]
% Here we ignore the dependence on item features $x_i$ for simplicity.

% To compute a prediction for content we



% Each user $u$ is a separate model weight vector $w_u \in \mathbb{R}^d$.

% Associated with each user $u$ and item $i$ are latent factors $w_u \in \mathbb{R}^d$ and $x_i \in \mathbb{R}^d$.
% The affinity of user $u$ has for item $i$ is then modeled as:
% \[
%   \text{affinity}(u,i) = w_u^T x_i  + \epsilon_{u,i}
% \]
% for $\epsilon_{u,i} \sim N(0,\sigma^2)$.

% Both the user factor $w_u$ and item factors $x_i$ are learned from data a




% While additional features may be used to capture knowledge about the user (\eg age) and the item (\eg genre) we restrict our attention to this simple model since it captures all the systems ideas in the later sections.

% Given observations about user affinities for a particular set of items we can infer the factors:
% \[
%   (w,x) = \arg \min_{w,x} \sum_{(u,i) \in \text{Ratings}}
%   \left( r_{ui} - w_u^T x_i  \right)^2 + \lambda \left(||w||_2^2 + ||x||_2^2 \right)
% \]

% Modern recommender systems employ machine learning models which are typically trained offline using iterative optimization algorithms and vasts amounts of data.



% function $f_u$ which maps an feature representation of an item $i$ to a real numbered score describing the affinity user $u$ has for item $i$.







% \subsubsection{Ensemble Methods}

% Many standard prediction and classification tasks can be expressed in the context of the GLM abstraction.
% In particular, by allowing $f(x,\theta)$ to be a collection of simpler machine learning techniques we can provide a range of model families





% \subsubsection{Recommender Systems}

% A popular class of data-products are recommender systems which target content to individuals by combining behavioral data (\eg ratings and clicks) with data describing users (\eg demographics), the items being considered (\eg content descriptions) and the context (\eg search queries).
% While there are many variations on the underlying model the majority of the recent developments have adopted a form of matrix factorization which we can cast within the Velox GLM abstraction.

% A separate model $w_u \in \mathbb{R}^d$ is constructed for each users $u$.
% The features $x \in \mathcal{X}$ describing each item $i$ (\eg color, price, etc...) in conjunction with ratings data are used to construct a latent feature representation $f(x_i) = \theta_i \in \mathbb{R}^d$ for each item.
% The affinity of user $u$ has for item $i$ is then modeled as:
% \[
%   \text{affinity}(u,i) = w_u^T \theta_i
% \]
% Given observations about user affinities (\eg ratings $r_{ui}$) for a particular set of items we can jointly infer the models for each user $w_u$ and the latent feature representation $\theta_i$ for each item by solving the following optimization problem:
% \[
%   (w,\theta) = \arg \min_{w,\theta} \lambda \left(||w||_2^2 + ||\theta||_2^2 \right) + \sum_{(u,i) \in \text{Obs}}
%   \left( r_{ui} - w_u^T \theta_i  \right)^2
% \]
% Here we ignore the dependence on item features $x_i$ for simplicity.

% To compute a prediction for content we



% Each user $u$ is a separate model weight vector $w_u \in \mathbb{R}^d$.

% Associated with each user $u$ and item $i$ are latent factors $w_u \in \mathbb{R}^d$ and $x_i \in \mathbb{R}^d$.
% The affinity of user $u$ has for item $i$ is then modeled as:
% \[
%   \text{affinity}(u,i) = w_u^T x_i  + \epsilon_{u,i}
% \]
% for $\epsilon_{u,i} \sim N(0,\sigma^2)$.

% Both the user factor $w_u$ and item factors $x_i$ are learned from data a




% While additional features may be used to capture knowledge about the user (\eg age) and the item (\eg genre) we restrict our attention to this simple model since it captures all the systems ideas in the later sections.

% Given observations about user affinities for a particular set of items we can infer the factors:
% \[
%   (w,x) = \arg \min_{w,x} \sum_{(u,i) \in \text{Ratings}}
%   \left( r_{ui} - w_u^T x_i  \right)^2 + \lambda \left(||w||_2^2 + ||x||_2^2 \right)
% \]

% Modern recommender systems employ machine learning models which are typically trained offline using iterative optimization algorithms and vasts amounts of data.



% function $f_u$ which maps an feature representation of an item $i$ to a real numbered score describing the affinity user $u$ has for item $i$.







% However, the success of recommender systems is not only determined by their ability to be trained at scale, but also to respond quickly to queries and incorporate new data as it becomes available.
% For example, a news recommendation service must be able to make recommendations about recent news articles and streaming music service needs to be able to respond to users feedback when selecting the next song to play.
% These later






% Because recommender systems are a popular class of data-product we will

% In this work we focus on the popular class of data-products broadly referred to as recommender systems.
% Recommender systems recommend content, ads, and products to individual users by combining behavioral data (\eg ratings and clicks) with data describing users (\eg demographics), the items being considered (\eg content descriptions) and the context (\eg search queries).
% Built on top of machine learning models, recommender systems are typically trained offline using large-scale cluster compute frameworks.
% The underlying models and sometimes their predictions are then materialized into a data-serving tier.








% Typically, data-products are built within large-scale analytics frameworks which are capable of training machine learning models.
% These models are then either mat

% Data-products are made possible by the development of systems to scale advanced techniques to vast amounts of data, data-products combine modeling and data








% \section{Recommendation Systems}

% The need to provide personalized experience has driven the design of a range of new technologies broadly referred to as recommendation systems.
% By combining vasts amounts of user data with recent developments in sophisticated statistical modeling techniques these systems are able to learn models describing individual users and content.

% At a high-level recommendation systems learn a scoring function from a user item pair to an affinity score which capture the user's affinity for the given item.





% While there are a wide range of modeling techniques employed in modern recommendation systems they all generally have a common form.




% for building such models we focus on a few of the basic elements that are representative of the design of recommender systems.

% At a high-level these systems model the affinity of users for a set of items as a function scoring the user and item pairs.







==> system.tex <==
%!TEX root = veloxms.tex

\section{\system System Design}

% Velox provides distributed model-serving and model-management
% as a service. Velox integrates easily with existing batch-analytics
% cluster compute frameworks such as Spark. By leveraging the significant computing
% power of these batch systems, Velox can delegate the heavy-lifting of
% model training and instead provides the serving and
% model management components of the system.

\subsection{Models in \system}

A model instance in \system has two components. The first is the user models $w$, represented as a
partioned table mapping a user ID \texttt{uid} to a vector of reals
$w_{\scriptscriptstyle \texttt{uid}} \in \mathbb{R}^d$. Because \system restricts the user models to a single linear model per user, there will always be a closed form solution to
updating the user model online.

The other component of \system is a \vmodel. by implementing the following interface:

\begin{lstlisting}

class VeloxModel {
  val name: String // user provided
  val state: Vector
  val version: Int // system provided



  // constructor
  def VeloxModel(state: Opt[Vector])

  // the featurization function
  def f(x: Data, materialized: Boolean) : Vector

  def retrain(f: (Data) => Vector,
              w: Table[String, Vector],
              newData: Seq[Data])
              => ((Data) => Vector, Table[String,Vector])

  def loss(y: Label,
           yPredict: Label,
           x: Data,
           uid: Long): Double
}

\end{lstlisting}

\vmodel has an optional constructor that takes a vector. This constructor can be used
to provide any global, immutable state (\ie $\theta$ from \secref{sec:background}) needed
during the featurization process. For example, this may be parameters for a featurization
function learned offline.

\vmodel next provides a function \texttt{f} representing the
feature transformation function. This may be a computation on some input data, as is the case
when the feature transformation is the computation of a set of basis functions on the input
data. Or this may be a lookup of the items latent features in a table, similar to
the table $w$ used to store the user models. The user indicates which of these two
methods is being used by specifying whether the features are materialized into
a table (in which case \texttt{materialized=True}), or are computed.  
The implementor specifies which of these strategies is in use to enable the system to
perform more effective performance optimization (see \secref{subsec:servepredictions}
for details). We intend to explore ways to automatically detect which approach is in use.
For example, by introspection of UDF byte-code to analyze data dependencies.

Finally, the user provides two functions, \texttt{retrain()} and \texttt{loss()} that
allow \system to automatically detect when models are stale and refresh them.
The \texttt{loss()} is evaluated every time new data is observed (\ie every time a
user model is updated) and if the loss starts to increase faster than a threshold value,
the model is detected as stale. Once a model has been detected as stale, \system
retrains the model offline using the cluster compute framework. \texttt{retrain()}
informs the cluster compute framework how to train this \vmodel, as well as where to find
the user interaction data needed for training. When offline training completes,
\system automatically instantiates a new \vmodel and new $w$, incrementing the version,
and transparently upgrading incoming prediction requests to be served with the newly
trained user-models and \vmodel.

This abstraction has several benefits. By treating all user models as linear weight vectors,
the system can always perform online updates for users, independent of the schema
implementation. Specifying whether a feature transformation has data dependencies
\system can decide on the best caching strategy. And providing support for both computational
and lookup-based feature transformations allows \system to
support a wide range of model implementations.
\dan{Discuss online updates here}


% \subsection{Making Predictions}
% % \label{subsec:servepredictions}
%
% \system provides two interfaces for serving predictions:
%
% \begin{lstlisting}
% def predict(s: ModelSchema, uid: Long, x: Data) : (Data, double)
% def best(s: ModelSchema, uid: Long, x: Set[Data],
%          max: (Seq[(Data, double)]) => (Data, double)) : (Data, double)
% \end{lstlisting}
% \texttt{predict()} serves point predictions for the provided user and item, returning
% the item and its predicted score. \texttt{best()} evaulates the best item from
% the provided set for the given \texttt{uid}. The \texttt{best()} function is useful
% in multiple settings. An application may want to support some prefiltering on the
% set of items to be recommended (\eg by whitelisting or blacklisting certain items)
% and can ask for predictions from \texttt{best()} to efficiently support this
% policy. And the multi-armed bandit techniques from \secref{sec:background} require
% the ability to choose \eg the second best prediction to serve to a user to
% improve the model quality faster.
%
% The primary expenses when serving predictions in \system are the cost of executing
% computationally expensive mathematical functions on the input (\eg the inner product
% of a user model and an item model to compute the prediction, or the featurization
% of a given input) and the cost of fetching remote data from over the network (\eg
% fetching an item's latent features stored on a remote machine). In other words,
% the primary expenses are lookups in either materialized feature transformation
% functions (fetching data) or computational feature transformation functions
% (expensive computation).
% These costs lead to two simple approaches to optimization: caching the
% results of computating basis functions for re-use, and efficiently partitioning and replicating distributed tables to limit remote data accesses. In addition, we can
% cache the actual prediction for a given (user,item) pair, another form
% of caching computations.
%
% The user model table $w$ is always fully materialized, and every prediction
% served is associated with a specific user $u$. Based on this observation, we partition $w$ across the \system cluster. Prediction requests are then routed based
% on their user ID to the server containing the corresponding partition of $w$.
% This partitioning serves a dual purpose. It ensures that lookups into $w$ can
% always be executed locally, and it provides a natural load-balancing scheme for
% distributing both serving load and the computational cost of online updates
% (see Section~\ref{subsec:onlineupdates}).
%
% When the feature transformation function \texttt{f} is materialized, corresponding to
% a lookup table, that table is also partitioned across the cluster. This means that
% evaluating \texttt{f} may involve an RPC to a remote machine containing
% the required key-value pair. However, while the number of items in the system
% may be large, item popularity often follows a power-law distribution with a heavy tail,
% meaning that many of these items are not frequently accessed, and a small subset of items
% are accessed very often. This suggests that caching the hot items on each machine, using a simple cache eviction strategy like LRU, will tend to have a high hit rate. And because
% these item models are only updated during the offline batch retraining, cached items are
% never overwritten and thus never need to be invalidated.
%
% When \texttt{f} is computational, caching the results of computing the basis functions
% can lead to similar benefits. If there are popular items, caching the item
% features both reduces prediction latency by eliminating the time to compute
% the potentially expensive featurization function, and reduces computational load on the
% serving machine which can lead to improved performance on the serving load.
%
% % However,
% % Caching
% % can lead to benefits if the popularity of items also follows a power-law like distribution,
% % but if the long-tail is too heavily weighted, then the benefits provided by a cache may
% % be small. However, if this cache is treated as replicated on a best-effort basis, then
% % the featurization computation for hot items can be amortized across the computational
% % resources of the entire cluster.
%
% The other computation that can be cached is the prediction itself, the result
% of $w_{\scriptscriptstyle \texttt{uid}} \times f(x)$. Caching the result of
% the prediction has the potential for the most increase in efficiency.
% In particular, repeated calls to \texttt{best()} with
% overlapping subsets will benefit from prediction caching.
%
%
%


% Making a prediction requires evaluating the trained model (or models) on the input and serving the result.
% Evaluating the model may be expensive, especially if several predictions are needed by the user-facing application to serve a result (\eg web page with personalized book recommendations).
% The system can either compute each prediction when a request for that prediction comes in, or it can remove the cost of computing the prediction from the hot-path of serving by predictions that have already been precomputed.
% Pre-computing all possible predictions is likely to be expensive and wasteful of computing resources.
% Most recommender systems have many more items than they will never recommend to a user than items that they will recommend, this imbalance is what drives the need for algorithmic recommendations in the first place.
% Thus, computing and storing all of those unneeded predictions is not helpful
% On the other hand, certain items may be recommended to a given user many times, meaning that the prediction for that item is needed frequently.
% In this case, having the precomputed prediction already, without having to compute it while trying to serve the prediction, can significantly improve serving latencies.
%
% This is not a new or novel problem, and one that is traditionally solved by caching "hot" predictions.
% However, there are two problems with using a naive caching strategy for this problem. The first is that serving predictions to the most active users is where the system sees the greatest benefit from caching, but the most active users are also the ones whose models
% are likely to be updated most frequently.
% Every time a model is updated, that invalidates any predictions computed from that model.
% The second problem is that every time the model is retrained offline, all cached predictions become invalidated and the whole system will suffer degraded performance until the cache is warmed up again.
%
% % Velox addresses the first issue by\dots
%
% When retraining the model offline, Velox also sends the cache membership list to the batch analytics framework.
% Once the model has been retrained, the cache is repopulated using the batch analytics system, so when Velox switches to the newly recomputed model, it can do so with a fully warmed up cache.
%
% In addition to caching results of a given prediction, we can exploit the formulation of a specific class of models called \emph{ensemble methods} to cache intermediate results.
% Ensemble methods compute a prediction as a weighted sum of the predictions of several
% underlying models that make up the ensemble. These models are shared across all users,
% while predictions are personalized by learning the correct model-weighting on a per-user
% basis. By caching the results of evaluating one of the underlying models in the ensemble
% on a given input, Velox amortizes that computation across future predictions on
% the item for all users. We use the same trick of warm-starting the cache when caching these
% intermediate predictions as well.


% key points: materialization (when, how much, where?). Caching (\eg cache/replicate frequently accessed/popular item models).
% Fuzzy prediction : Ensemble methods
% how can we share predictions/computation for similar items (leverage statistical properties
% of model). Model size.

\subsection{Online and Offline Training}
\label{subsec:onlineupdates}

\dan{Need a section about online updates}

In addition to performing lightweight, online updates to user models,
\system automatically determines when the models are too stale and
triggers the batch analytics system to recompute the models offline.
This offline recomputation yields new \vsets that are colocated with the old
\vsets (\ie partitioning functions do not change). Switching from the old to
the new model means updating the pointers to the new \vsets (\system internally
stores a hash-table that contains the current location and partitioning function
of each explicit \vset), and invalidating any cache entries that are now out of date.


\dan{Is this a viable proposal for detecting model staleness?}
To determine when the model is too stale, the system periodically evaluates model
quality on a small subset of both new and old items with known ratings. If the
online-updates no longer improve the quality of the model even as new information
comes in, \system determines that the models are stale and should be refreshed offline.


key points:
How does doing online updates affect resource utilization (do we see serving latencies spike when we turn on online updates)?

Detect when model is stale, should be retrained offline. How to switch from old to new model.
Cache-invalidation/what to do about pre-materialized predictions. Can we warm up the cache?
How do we manage multiple models? Multi-armed bandit.

% \subsection{Distributed Serving}
%
% Velox has been designed from the beginning to operate in a distributed environment by effectively partitioning both the serving load and the underlying model and data storage. At the heart of a recommender system is making predictions for a specific user.
% User recommendations use
% predictions from that user's model, and are independent of all other user models. By
% distributing user models across the Velox cluster and routing requests for a given user to
% the correct machine, we ensure data locality for both low-latency predictions and
% load balancing of the online update computations. To reduce network delays for frequently
% accessed item models, we cache models for hot items on a per-server basis. These models
% are read-only between offline updates, so they only get evicted from the cache when they
% cool down.
%
% When dealing with shared ensemble models, the best partitioning strategy is less obvious.
% However
%
% Key points:
% Distribution (\eg partition user models and
% direct requests for that user to the correct velox instance/machine).
% Data partitioning and replication
% Model consistency? (Here can we take advantage of statistical properties...)


\subsection{Integration with Analytics Frameworks}

Velox requires a way to share both raw data and trained models between the serving layer
and the batch analytics framework (\eg Spark).
Velox must be able to read the models trained offline and write to them as it performs online updates.
It must also be able to write raw data to log files to record interactions with the user-facing application.
The batch analytics framework must be able to read the raw data from Velox's logs to train the model, and it must be able to write the offline-trained models for Velox to read.
To facilitate this data sharing, Velox leverages the Tachyon in-memory file system which was designed for exactly this purpose. Specifically, we leverage an experimental new feature
of Tachyon that implements an append-only key-value store with an index for efficient
random access.

Velox runs co-located with a Tachyon cluster, independent of the cluster-compute framework.
Running colocated with the primary data storage system, but independent from the batch analytics system, presents several advantages.
Cluster compute systems perform compute-intensive operations, especially when training machine-learning models, and performing these computations on the same hardware as a serving system with low-latency requirements can lead to serious performance degradation when retraining the models
By using Tachyon as the interface between the systems, it allows for significant flexibility in the choice of cluster-compute system and the deployment configuration
As long as the system can read and write from HDFS and jobs can be monitored remotely (requirements that virtually every cluster-compute framework designed to be deployed to an AWS-style cloud meets), Velox can use it for offline training
Furthermore, batch analytics systems generally require ownership of the full dataset, so regardless of where the input data is located, it will need to be copied into the system.
We force the over-the-network data transfer to happen during the offline-training step because this step is much less latency sensitive, and can amortize some of the transfer costs by doing it in bulk.

In addition to sharing data, Velox must be able to trigger full recomputation of the models
via offline training. Once Velox has detected that the model is too stale
and should be fully-trained, it simply connects to the cluster-compute
master and tells it to re-run the computation, as well as telling it the
location of the logs containing the latest user interaction data.














% \section{Challenges and Opportunities}
%
% We start by outlining some of challenges in building a model-serving system.
% Some of these issues will sound familiar to any databases student, and have been well-studied in the databases community.
% In these cases, we plan to leverage the existing body of work and study which parts apply (and perhaps which do not) to this new domain.
% Others are newer, more closely tied with the math underlying the model learning and prediction processes.
% Here, we hope to develop a principled understanding of the impact the design of models and features has on the system (both in terms of design and performance).
%
%
% \subsection{Materialization}
%
% The first challenge in this space is how to partially materialize predictions for faster prediction queries. There are several choices to be made both in determining what to materialize, and determining the granularity of materialization.
%
% In the simple cases we examine in this paper, the result of querying a model-serving system is either a single prediction (e.g. a regression score) or a list of the top-k predictions.
% Materializing predictions presents an obvious choice. However, in many domains, the vast majority of predictions will never be needed, so fully materializing the prediction set leads to wasted space and addititional IO and search costs (whether from disk, network, or main-memory), as well as a huge wasted CPU cost from making predictions (doing dot-products) that will never be needed. Determining what subset of predictions should be materialized to balance improved performance with judicious space usage will be one simple way to improve performance.
%
% As previously discussed, a model is some function $f(\text{features}(x)) \rightarrow \text{prediction}$, where $x$ is the query input (\eg some profile information about a user).
% The featurization process presents another opportunity for materialization.
% The actual features to use are typically selected ahead of time in a process with a human in the loop, and then represented as static functions $f_i(x)\ \mbox{for}\ i=1, \ldots, k$ to compute the $k$ features.
% Thus, computing many predictions for the same input can lead to significant recomputation of features.
% Caching the features for a given input will certainly improve performance, particularly in the common case when we are making predictions using several models.
% The more interesting case is how to cache the $(\text{input},\text{feature})$ mapping pairs to be shared between different inputs. In some cases, the relevant part of the input may be categorical data (\eg age, zipcode) in which case it might make sense to explicitly enumerate all input-output pairs of the function in a lookup table rather than computing them on-demand. However, as the cardinality of the possible inputs grows, there will be cross-over point where it is more efficient to compute the feature function rather than trying to lookup the mapping in a materialized table. Because features are an approximation of the dataset, while they must be accurate to be useful, there is some flexibility with exactly which features are chosen. In fact, this flexibility is already used by data-scientists during the feature selection process (\eg choosing features for statistical usefulness vs. real-world explanatory power, etc \cite{Zhang2014}). We hope to exploit this flexibility to examine the tradeoffs in caching and sharing features, cost of computing features, and prediction quality.
%
% Related to this tradeoff is the possibility of fuzzy predictions. Find nearest materialized prediction and if the feature vectors of the two inputs are close enough, use that prediction, otherwise make the prediction with the provided input and cache the results.
%
%
% \subsection{Managing multiple models}
%
% In many cases, there may be several models available to make predictions.
% Which model to use for a given prediction may vary based on recently observed user behavior or other temporal components.
% For example, an online shopping website may train (offline) several different models for each user, that describe different ways that user interacts for the website.
% They may have a model that describes how that user searches for books and music (\ie describes this users media consumption habits).
% They may have another that models how they buy household supplies and toiletries, another for clothes shopping, and yet another that models how this user searches for gifts.
% While all these models are based on the same user, the shopping site has no way to predict ahead of time which of these models best describes the users actions for a given shopping session.
% One option would be to show a mixture of the predictions of each model (indeed, that is often the solution taken today).
% But even better would be to learn the correct weight to give predictions from each model as the user interacts with the website in a given shopping session.
% This simple, online learning task can dramatically improve both the users experience and the websites revenue by providing better recommendations.
%
% In order to support this, the serving system must be able to support storing and querying predictions from multiple models.
% The system must also be able to update the weight distribution for the models as the user continues to interact with the system.
% And it must also be able to identify when an individual model for a user is too stale and should be retrained, as well as when the model distribution for the user no longer accurately models their behavior (maybe the user had a baby and now buys baby supplies, but there is no model to describe how the user buys baby supplies).
% The system should be able to automatically detect this situation on a per-user basis and provide this feedback to the offline training system.
%
% \subsection{Online Updates}
%
% In addition to updating the relative weights of our ensemble of models, prediction quality can be improved by updating the models themselves to adapt to new user behavior.
% Consider a recommender system for an online radio application where users can select a radio station and indicate that they like or dislike a song (or remain neutral).
% If a user selects a new radio station and starts liking or disliking songs, the recommender system can provide better personalization if they can take into account these new user reviews (\ie this additional insight into this users preferences), rather than relying on the model trained on data that was not able to incorporate these preferences.
% At the same time, any model updates must be fast because the are most useful as the user is still interacting with the system.
%
% In order to perform online updates in a low-latency serving system, there are a few considerations that must be accounted for.
% The first is model staleness.
% Retraining the user model after every new rating comes in may be inefficient (especially in a highly concurrent setting).
% The system needs to balance model freshness and effective resource utilization by choosing a batch size for the online updates.
% \dan{discuss the different performance parameters here, for example, might need to read other rating info from disk, might need to invalidate/update materialized predictions, etc.}.
%
% \subsection{Standard Interface}
%
%
% \section{The design of \system}
%
% In this section, we present \system and discuss the design decisions behind

